On Dependent Dirichlet Processes for General Polish Spaces

We study Dirichlet process-based models for sets of predictor-dependent probability distributions, where the domain and predictor space are general Polish spaces. We generalize the definition of dependent Dirichlet processes, originally constructed on Euclidean spaces, to more general Polish spaces. We provide sufficient conditions under which dependent Dirichlet processes have appealing properties regarding continuity (weak and strong), association structure, and support (under different topologies). We also provide sufficient conditions under which mixture models induced by dependent Dirichlet processes have appealing properties regarding strong continuity, association structure, support, and weak consistency under i.i.d. sampling of both responses and predictors. The results can be easily extended to more general dependent stick-breaking processes.

==> global_definitions.tex <==
%   
%   =========   USEFUL GLOBAL DEFINITIONS

%   ---------   FORMATTING
%               commands
\newcommand{\wh}[1]{\widehat{#1}}                           % alias for widehat
\newcommand{\ol}[1]{\overline{#1}}                          % alias for overline
\newcommand{\bmtx}[1]{\begin{bmatrix} #1 \end{bmatrix}}     % alias for bracketed matrices
%               definitions
\def\sumsub{\sum\nolimits}                                  % sum with no subscript
\def\limsub{\lim\nolimits}                                  % limit with no subscript
\def\supsub{\sup\nolimits}                                  % supremum with no subscript
\def\infsub{\inf\nolimits}                                  % infimum with no subscript
\def\QED{\flushright Q.E.D.}                                % for proofs

%   *********   CME108 NOTES
\newcommand{\fl}[1]{\msf{fl}(#1)}
\newcommand{\binop}[2]{#1 \msf{\phantom{.}op\phantom{.}} #2}

%   *********   NUMBER SYSTEMS AND SPECIAL SYMBOLS
\def\N{\mathbb{N}}              		%	natural numbers
\def\Q{\mathbb{Q}}              		%	rational numbers
\def\R{\mathbb{R}}              		%	real numbers
\def\Z{\mathbb{Z}}              		% 	integers
\def\C{\mathbb{C}}              		%	complex numbers
\def\Rp{\mathbb{R}_{+}}         		%	non-negative real numbers
\def\Rsp{\mathbb{R}_{>}}        		%	strictly positive real numbers
\def\1i{\msf{i}} 						%	imaginary unit
\def\eps{\varepsilon} 					%	shorthand for \varepsilon
\def\vphi{\varphi} 						%	shorthand for \varphi
\def\real{\operatorname{Re}} 			%	real part
\def\imag{\operatorname{Im}}		    %	imaginary part
\def\comp{\circ} 						% 	function composition
\def\minone{-1} 
\newcommand{\conj}[1]{\overline{#1}} 	%	complex conjugate\\
\def\Matlab{\textsc{Matlab}} 			% 	MATLAB(TM)
\def\sreal{		\mfr{r}} 				% 	real part (subscript notation)
\def\simag{ 	\mfr{i}} 				% 	imaginary part (subscript notation)

%	*********   MATH FORMATTING
\newcommand{\vc}[1]{{\boldsymbol #1}}   %   vector/matrix symbols
\newcommand{\mc}[1]{\mathcal{#1}} 		%	\mathcal{} 		(caligraphic)
\newcommand{\mbb}[1]{\mathbb{#1}} 		% 	\mathbb{} 		(blackboard)
\newcommand{\mbf}[1]{\mathbf{#1}} 		% 	\mathbf{} 	 	(boldface)	
\newcommand{\mfr}[1]{\mathfrak{#1}} 	% 	\mathfrak{} 	(fraktur)
\newcommand{\msf}[1]{\mathsf{#1}} 		% 	\mathsf{} 		(serif)
\newcommand{\mrm}[1]{\mathrm{#1}} 		%   \mathrm{} 		(plain text)
\newcommand{\mtt}[1]{\mathtt{#1}} 		% 	\mathtt{} 		(typewriter)

% 	********* 	CALCULUS
\renewcommand{\exp}[1]{\ensuremath{\,\textrm{e}^{#1}\,}} 	% 	exponential function
\def\Exp{\mathrm{exp}} 										% 	exponential function (Lie groups)
\def\ind{\mbb{I}} 											% 	indicator function (symbol)
\def\idx{\mc{I}}                                            %   index set
\def\sinc{\operatorname{sinc}}                              %   sinc function
\def\hot{\mathrm{h.o.t.}}
\def\sign{\operatorname{\mathbf{sign}}}                     % 	sign
\def\compO{O}                                               % 	Big-O
\def\compo{o}                                               % 	Little-O
\def\compT{\Theta}                                          % 	Theta
\newcommand{\floor}[1]{\lfloor #1 \rfloor}		        	%	floor function
\newcommand{\ceil}[1]{\lceil #1 \rceil}                 	%	ceiling function
\newcommand{\sublev}[2]{\operatorname{\mbf{lev}}_{\leq #1}(#2)}

% 	*********   SET THEORY AND TOPOLOGY
\def\rel{   \operatorname{\mbf{rel}}} 			% 	PREFIX: relative
\def\topint{\operatorname{\mbf{int}}}			% 	interior 			(topological)
\def\topcl{ \operatorname{\mbf{cerr}}} 			% 	closure 			(topological)
\def\topbd{ \operatorname{\mbf{fr}}} 			%	boundary 			(topological)
\newcommand{\eqclass}[1]{[#1]} 					%	equivalence class
\newcommand{\Leqclass}[1]{\left[#1\right]} 		%	equivalence class	(large)


% 	*********	ANALYSIS
\newcommand{\iprod}[2]{\langle #1,\, #2\rangle}	            % 	inner product
\newcommand{\Liprod}[2]{\left\langle#1,\, #2\right\rangle}	% 	inner product 		(large)
\newcommand{\nrm}[1]{\|#1\|} 								% 	norm
\newcommand{\Lnrm}[1]{\left\|#1\right\|} 					% 	norm 				(large)
\newcommand{\seq}[3]{\{#1\}_{#2}^{#3}} 						% 	sequence
\newcommand{\Lseq}[3]{\left\{#1\right\}_{#2}^{#3}} 			% 	sequence 			(large)
\newcommand{\set}[1]{\{#1\}} 								% 	set
\newcommand{\Lset}[1]{\left\{#1\right\}} 					%	set					(large)
\newcommand{\pset}[1]{(#1)} 								% 	set
\newcommand{\Lpset}[1]{\left(#1\right)} 					%	set					(large)
\newcommand{\bset}[1]{[#1]} 								% 	set
\newcommand{\Lbset}[1]{\left[#1\right]} 					%	set					(large)
\newcommand{\feval}[2]{#1|_{#2}} 							% 	function evaluation
\newcommand{\Lfeval}[2]{\left.#1\right|_{#2}} 				% 	function evaluation (large)
\newcommand{\restr}[2]{#1|_{#2}} 							% 	restriction
\newcommand{\Lrestr}[2]{\left.#1\right|_{#2}} 				% 	restriction 		(large)
\newcommand{\lieder}[1]{\mathcal{L}_{#1}}

\def\loc{ 	\textrm{loc}} 					% 	local
\def\lipcst{\operatorname{\mrm{Lip}}}       %   Lipschitz constant
\def\ker{  \operatorname{\mbf{null}}} 		% 	kernel
\def\range{\operatorname{\mbf{ran}}}		%	range
\def\im{\operatorname{\mbf{im}}}		%	range
\def\dom{\operatorname{\mbf{dom}}}		    %	domain
\def\rank{ \operatorname{\mbf{rank}}} 		% 	rank
\def\dim{  \operatorname{\mbf{dim}}} 		% 	dimension
\def\graph{\operatorname{\mbf{graph}}} 		% 	graph
\def\vspan{\operatorname{\mbf{gen}}} 		% 	span
\def\dist{ \operatorname{\mbf{dist}}} 		% 	distance
\def\div{  \operatorname{\mbf{div}}} 		% 	divergence
\def\supp{ \operatorname{\mbf{supp}}} 		% 	support
\def\supess{\operatorname{supess}}                  % essential support
\def\diam{ \operatorname{\mbf{diam}}} 		% 	diameter
\def\graph{\operatorname{\mbf{graph}}} 		% 	graph
\def\id{   \operatorname{id}} 				% 	identity
\def\proj{ \operatorname{\mbf{proj}}} 			%  	projection
\def\prox{ \operatorname{prox}} 			% 	proximal map
\def\evmap{\operatorname{\mbf{ev}}}         %   evaluation map

% 	*********	CONVEX ANALYSIS
\def\epi{    \operatorname{\mbf{epi}}} 		% 	epigraph
\def\cvxdom{ \operatorname{\mbf{dom}}} 		% 	convex domain
\def\aff{    \operatorname{\mbf{aff}}}		% 	affine hull
\def\cvxhull{\operatorname{\mbf{conv}}}		%	convex hull
\def\relint{ \rel\topint} 					% 	relative interior
\def\cone{ 	 \operatorname{\mbf{cone}}} 	% 	conic hull
\def\cvxdual{\star} 						% 	convex dual

% 	*********	OPTIMIZATION
\def\opt{\star} 		% 	optimum

% 	*********	LINEAR ALGEBRA
\def\diag{  \operatorname{\mbf{diag}}}		% 	diagonal
\def\trace{ \operatorname{\mbf{trace}}} 	% 	trace
\def\det{   \operatorname{\mbf{det}}}       %   determinant
\def\svd{   \text{svd}}                     %   singular-value decomposition
\def\ph{    \operatorname{\mbf{ph}}} 		% 	phase
\def\op{    \operatorname{\mrm{op}}} 		% 	operator
\def\vander{\operatorname{\msf{V}}}         % Vandermonde matrix

%   *********   PROBABILITY AND STATISTICS
\def\Unif{  \operatorname{\mathsf{unif}}}   %   uniform distribution
\def\mse{	\operatorname{\mrm{MSE}}} 		% 	mean-squared error
\def\sure{	\operatorname{\mrm{SURE}}} 		% 	SURE
\def\ev{    \operatorname{\mbf{E}}} 		% 	expected value
\def\var{   \mbf{V}} 						% 	variance
\def\cov{   \operatorname{\mbf{Cov}}}       %   covariance
\def\prob{  \mbf{P}} 						% 	probability
\newcommand{\est}[1]{\hat{#1}} 				% 	estimator
\def\iid{\mrm{iid}} 						% 	i.i.d.: independent, identically distributed
\def\Poisson{\textsc{Poisson}} 			    % 	Poisson distribution

\def\paral{\parallel}
\def\symmtx{\operatorname{\mathsf{Sym}}}
\def\skewmtx{\operatorname{\mathsf{Skew}}}
\def\orthmtx{\operatorname{\mathsf{O}}}
\def\unitmtx{\operatorname{\mathsf{U}}}
\def\pergrp{\operatorname{\textbf{S}}}
\def\diagmtx{\operatorname{\mathbf{Diag}}}

% 	*********	GROUP THEORY
\def\stab{\mathsf{Stab}}
\def\orbit{\mathsf{Orbit}}

%   *********   COMMON ENVIRONMENTS
%\theoremstyle{theorem}
%\newtheorem*{mthm}{Theorem}
%\theoremstyle{theorem}
%\newtheorem*{mlem}{Lemma}
%\theoremstyle{mcor}
%\newtheorem*{mcor}{Corollary}
%\theoremstyle{remark}
%\newtheorem*{mrem}{Remark}

%   *********   OPTIMIZATION TEMPLATE
%\begin{equation}
%    \label{xx:yy}
%    \begin{aligned}
%    & \underset{[variable]}{\text{minimize}}
%    & & [objective]\\
%    & \text{subject to}
%    & & [constraint a]\\
%    & & & [constraint b]
%    \end{aligned}
%\end{equation}

%   *********   EQUATION TEMPLEATE
%\begin{equation}
%\begin{aligned}
%    [OPERATOR] &= [SOURCE]      && \qquad [DOMAIN],\\
%    [BOUNDARY] &= [CONDITION]   && \qquad [DOMAIN]
%\end{aligned}
%\end{equation}
